Fishr: Invariant Gradient Variances for Out-of-Distribution Generalization

Learning robust models that generalize well under changes in the data distribution is critical for real-world applications. To this end, there has been a growing surge of interest to learn simultaneously from multiple training domains - while enforcing different types of invariance across those domains. Yet, all existing approaches fail to show systematic benefits under controlled evaluation protocols. In this paper, we introduce a new regularization - named Fishr - that enforces domain invariance in the space of the gradients of the loss: specifically, the domain-level variances of gradients are matched across training domains. Our approach is based on the close relations between the gradient covariance, the Fisher Information and the Hessian of the loss: in particular, we show that Fishr eventually aligns the domain-level loss landscapes locally around the final weights. Extensive experiments demonstrate the effectiveness of Fishr for out-of-distribution generalization. Notably, Fishr improves the state of the art on the DomainBed benchmark and performs consistently better than Empirical Risk Minimization. Our code is available at https://github.com/alexrame/fishr.

==> pictures/deprecated/cov_efim_fim_h.tex <==
\begin{wrapfigure}[18]{hR!}{0.34\textwidth}
    \vspace{-2.0em}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/model/files/vrexfishrhessian.jpg}%
    \vspace{-0.5em}
    \caption{\textbf{Colored MNIST dynamics}, where $\mathcal{E}=\{90\%,80\%\}$. Details in Appendix \ref{appendix:cmnistdetails}.
    At epoch 190, $\lambda$ strongly steps up: then the Fishr regularization from Eq.~\ref{eq:fishrreg} matches the domain-level gradients covariances ($\mC_{90\%}$ and $\mC_{80\%}$, blue line).
    Critically, Fishr also reduces the distance between the two domain-level Hessians ($\mH_{90\%}$ and $\mH_{80\%}$, green line).}
    \label{fig:vrexfishrhessian}%
\end{wrapfigure}

% CUDA_VISIBLE_DEVICES=7 python -m domainbed.scripts.train_cmnist_hessian --algorithm fishr --n_restarts 1 --output_size 1


==> pictures/deprecated/expes/cmnist_irm_labelflipping_vs_acc.tex <==
% from 0 to 0.25 proba of error in train/test
% how accuracy evolves


==> pictures/deprecated/expes/lambda_vs_acc.tex <==
\begin{figure}[!h]%
    \centering%
    \includegraphics[width=0.8\linewidth]{pictures/expes/files/vlcs_db_env2_l_vs_acc.png}
    % pictures/expes/files/cmnist_db_env2_mmdl_vs_acc.png
    \caption{
        % \textbf{Domainbed version of the Colored MNIST dataset},  when the training domains are $\mathcal{E}=\left\{90\%,80\%\right\}$.
        % \textbf{TerraIncognita}, when the training domains are $\mathcal{E}=\left\{L100, L38, L43\right\}$ and the test set is $L46$.
        \textbf{Experiments on VLCS in DomainBed}, when the training domains are $\mathcal{E}=\left\{V, L, C\right\}$ and the test set is $S$.
        These 120 points are obtained using 2 DomainBed sweeps (one where $\lambda\sim10^{\text {Uniform}(1,4)}$ and the other where $\lambda\sim10^{\text {Uniform}(1,5)}$), with 20 trials each and 3 different seeds.
        While sampling $\lambda$ from $10^{\text {Uniform}(1,5)}$ performs better with 'Oracle' model selection (72.7 versus 72.0 for $10^{\text {Uniform}(1,4)}$), it performs worse on 'Training' (71.8 versus 73.9).
        In particular, $\lambda=$
        Excessively high $\lambda$s generally decrease training-domain validation accuracies but may perform well on the test.
        The high variability in accuracy is increased by the randomness of the other hyperparameters values (\textit{e.g.} learning rate, batch size, \dots).}
    % on CIFAR-100 with a WRN-28-10 and $b_r\scalemath{1.}{=}2$.}%
    \label{fig:lambda_vs_acc}%
    % \vspace{-0.5em}%
\end{figure}%



% oracle
% Fishrv15              & 97.9 $\pm$ 0.3 & 65.7 $\pm$ 0.6 & 72.7 $\pm$ 0.6 & 76.4 $\pm$ 0.6 & 78.2          \\
% Fishr              & 97.8 $\pm$ 0.2 & 68.1 $\pm$ 0.4 & 72.0 $\pm$ 1.0 & 75.5 $\pm$ 0.9 & 78.4             \\
% training
% Fishr15            & 98.3 $\pm$ 0.2 & 64.8 $\pm$ 0.6 & 71.8 $\pm$ 1.0 & 76.2 $\pm$ 0.4 & 77.8         \\
% Fishr              & 98.4 $\pm$ 0.1 & 64.4 $\pm$ 0.4 & 73.9 $\pm$ 1.1 & 76.8 $\pm$ 0.7 & 78.4             \\


==> pictures/deprecated/hessianl2cos.tex <==
\begin{wrapfigure}[28]{hR!}{0.38\textwidth}
    \vspace{-10.0em}
    \centering
    \includegraphics[width=1.0\linewidth]{pictures/model/files/hessianl2cos.jpg}%
    \caption{\textbf{Hessians dynamics on Colored MNIST with Fishr}. At epoch 190, $\lambda$ steps us and then domain-level Hessians take similar directions (high cosine similarity) and norms.}
    \label{fig:hessianl2cos}%
    \vspace{1.0em}
    \includegraphics[width=1.0\linewidth]{pictures/model/files/vrexfishrhessian_forerm.jpg}%
    \caption{\textbf{Dynamics on Colored MNIST with ERM}: $\lambda=0$ during the whole training. The distance between domain-level Hessians keeps increasing.}
    \label{fig:cov_h_erm}%
    \vspace{1.0em}
    \includegraphics[width=1.0\linewidth]{pictures/model/files/fishrrex.jpg}%
    \caption{\textbf{Risks dynamics on Colored MNIST with Fishr}. At epoch 190, $\lambda$ steps us and then domain-level empirical risks become similar.}
    \label{fig:fishrrex}
\end{wrapfigure}


==> pictures/model/fig_propconsistency.tex <==
% \begin{wrapfigure}[12]{h}{0.40\textwidth}
%     % \vspace{-2em}
%     \centering
%     \includegraphics[width=1.0\linewidth]{pictures/model/files/demonstration.png}%
%     % \vspace{-0.5em}
%     \caption{\textbf{Loss landscapes}.
%     }
%     \label{fig:demo}%
%     % \vspace{-1.0em}
% \end{wrapfigure}

\begin{figure}[h]
    \centering
    \includegraphics[width=.8\linewidth]{pictures/model/files/demonstration.png}
    % \vspace{-0.2em}
    \caption{\textbf{Loss landscapes}.}
    \label{fig:propconsistency}
\end{figure}

==> pictures/pseudocode.tex <==
\begin{algorithm}[H]%
    \DontPrintSemicolon%
    \tcc{Setup}%
    \KwParams{Network $f_{\theta}$, made of a deep features extractor $\Phi_{\phi}$ and a dense linear classifier $w_{\omega}$, randomly initialized.}
    \KwInput{
    Observations $\mathcal{D}_{e}=\left\{\left(\vx_{e}^{i}, \vy_{e}^{i}\right)\right\}_{i=1}^{n_{e}}$ for domains $e\in\mathcal{E}$,
    regularization weight $\lambda$, warmup iteration $i_{\text{warmup}}$ and exponential moving average speed $\gamma$, batch size $b_s$, optimizer $g$, learning rate $l_r$.}%
    \tcc{Training Procedure}%
    Initialize moving averages: $\forall e\in\mathcal{E}, \vv_e^{\text{mean}}\gets 0$\\
    \For{$\text{iter}$ \textbf{from} $1$ \textbf{to} \#iters} {%
    \tcc{Step 1: standard ERM procedure}%

    \For{$e\in\mathcal{E}$} {%
    Randomly select batch: $\{(\vx_{e}^{i}, \vy_{e}^{i})\}_{i\in \mathcal{B}}$ of size $b_s$\\
    Compute predictions: $\forall i\in \mathcal{B}, \hat{\vy}_e^{i} \gets f_{\theta}(\vx_{e}^i)$\\
    Compute domain empirical risk: $\mathcal{R}_{e}(\theta) \gets \sum_{i\in \mathcal{B}} \ell\left(\hat{\vy}_e^{i}, \vy_{e}^{i}\right)$
    }
    $ \mathcal{L}(\theta)=\frac{1}{|\mathcal{E}|} \sum_{e\in\mathcal{E}} \mathcal{R}_{e}(\theta)$\\
    \tcc{Step 2: gradient variances in classifier}
    \For{$e\in\mathcal{E}$} {%
    Compute individual gradients in $w_{\omega}$ with BackPACK: $\forall i\in \mathcal{B}, \vg_{e}^{i} \gets \nabla_{\omega} \ell\left(\hat{\vy}_e^{i}, \vy_{e}^{i}\right)$\\
    Compute domain-level gradient variances:
    $\vv_e^{\text{iter}} = \frac{1}{b_s}\sum_{i\in\mathcal{B}}(\vg_{e}^{i}-\frac{1}{b_s}\sum_{j\in\mathcal{B}} \vg_{e}^{j})^2$\\
    Moving average: $\vv_e \gets \gamma \vv_e^{\text{mean}}+(1-\gamma)\vv_e^{\text{iter}}$\\
    Update moving average: $\vv_e^{\text{mean}} \gets detach(\vv_e)$\\
    Correction: $\vv_e \gets \frac{1}{1-\gamma}\vv_e$ (see Appendix \ref{appendix:domainbeddetails})\\
    }

    \uIf{$\text{iter} \geq i_{\text{warmup}}$}{
    Average the domain-level variances: $\vv=\frac{1}{|\mathcal{E}|}\sum_{e\in\mathcal{E}}\vv_{e}$\\
    Compute the regularization loss: $\mathcal{L}_{\text{Fishr}}(\theta)=\frac{1}{|\mathcal{E}|}\sum_{e\in\mathcal{E}}\sum_{\pi\in\omega}|\vv_e^{\pi} - \vv^{\pi}|^2$\\
    $   \mathcal{L}(\theta) \mathrel{{+}{=}} \lambda \mathcal{L}_{\text{Fishr}}(\theta)$
    }
    \tcc{Step 3: gradient descent}%
    Backpropagate gradients: $\theta \gets g\left(\text{gradient}=\nabla_{\theta} \mathcal{L}(\theta), \text{learning rate}=l_r\right)$\\
    }%
    \caption{Training procedure for Fishr on DomainBed}%
    \label{pseudocode}
\end{algorithm}%


==> sections/04_implem.tex <==
\section{Scalable implementation}

\label{model:implem}
% Our goal
We now describe three implementation choices that make Fishr easily applicable at almost the same computational costs as ERM.

\textit{First}, to reduce the memory overhead, we only consider the gradients in the \textbf{final linear classifier} $w_{\omega}$: $\vg_{e}^{i}=\nabla_{\omega}\ell\left[w_{\omega}\left(\Phi_{\phi}(\vx_{e}^i)\right),\vy_{e}^{i}\right]$. It's worth noting that these gradients in $\omega$ depend on $\Phi_{\phi}$.
We ignore the gradients in the features extractor $\Phi_{\phi}$ because low-level layers may need to adapt to domain-dependent peculiarities: on the contrary, invariance in high-level features is more critical. This intuition --- strengthened in Appendix \ref{appendix:iga} --- is classical in unsupervised domain adaptation \citep{ganin2016domain} and for computing influence functions \citep{ye2021out,pezeshkpour2021n}. This is also consistent with concurrent approaches in OOD generalization that seek invariant predictors \citep{arjovsky2019invariant,krueger2020utofdistribution}.
Moreover, if we used all weights $\theta = \omega \oplus \phi$ to compute $\mC$, the invariance in  $w_{\omega}$ would get overshadowed by $\Phi_{\phi}$ due to $|\omega| \ll |\phi|$.

\textit{Second},
we only use \textbf{the gradient variance} --- \textit{i.e.}, the diagonal of the covariance matrix $\operatorname{Diag}(\mC)$ --- to scale down the number of targeted components from $|\omega|^2$ to $|\omega|$. This is similar to AND-mask \citep{parascandolo2021learning} which only considers $\operatorname{Diag}(\mH)$ based on the empirical evidence \citep{becker1988improving,adolphs2019ellipsoidal,NEURIPS2020_d1ff1ec8} that Hessians are diagonally dominant at the end of training. More generally, this Hessian diagonal approximation is common in optimization \citep{series/lncs/LeCunBOM12,kingma2014adam}, continual learning \citep{kirkpatrick2017overcoming} and pruning \citep{e9ee2143e19d49cf9cbe8861950b6b2a,Theis2018a}.
Since we highlighted empirical similarities between $\mH$ and $\mC$, we ignore the off-diagonal parts in $\mC$.
This is also motivated by the critical importance of $\operatorname{Tr}(\mH)$ \citep{yao2020pyhessian} and $\operatorname{Tr}(\mC)$ \citep{jastrzebski2021catastrophic} to analyze the generalization properties of DNNs.
In Appendix \ref{appendix:offdiag}, we empirically observe that ignoring or not the off-diagonal parts performs similarly on Colored MNIST.
Future work could consider refined interactions between weights using K-FAC approximations \citep{heskes2000natural,10.5555/3045118.3045374}.
% We validate the quality of this approximation in Appendix \ref{appendix:ablation}.
In summary, we match the \textbf{variances of gradients for each weight in the classifier}:
\begin{equation}
% \vspace{-0.3em}
    \mathcal{L}_{\text{Fishr}}(\theta)=\frac{1}{|\mathcal{E}|}\sum\nolimits_{e\in\mathcal{E}}\sum\nolimits_{\pi\in\omega}|\vv_e^{\pi} - \vv^{\pi}|^2,
\end{equation}
where the scalar $\vv^{\pi}=\frac{1}{|\mathcal{E}|}\sum_{e\in\mathcal{E}}\vv_{e}^{\pi}$ averages the domain-level variances per classifier weight $\pi$:
\begin{equation}
% \vspace{-0.3em}
    \vv_e^{\pi} = \frac{1}{n_{e}-1}\sum\nolimits_{i=1}^{n_{e}}(\nabla_{\pi}\ell\left[w_{\omega}\left(\Phi_{\phi}(\vx_{e}^i)\right),\vy_{e}^{i}\right]-\frac{1}{n_{e}}\sum\nolimits_{j=1}^{n_{e}} \nabla_{\pi}\ell\left[w_{\omega}\left(\Phi_{\phi}(\vx_{e}^j)\right),\vy_{e}^{j}\right])^2.
    \label{eq:variance}
\end{equation}

\textit{Third}, PyTorch \citep{NEURIPS2019_9015} is optimized only to compute the batch-averaged gradients.
% On the contrary, we need the loss gradients .
Fortunately, the recent BackPACK \citep{dangel2020backpack} package keeps additional information from first- and second-order derivatives.
Notably, it supports efficient computation of individual gradients, sample per sample, from a batch at almost no time overhead. Moreover, the \textit{DiagHessian} method in BackPACK computes the Hessian diagonals, and is used for analysis in Table \ref{table:hessianermfishr} and Fig.\ \ref{fig:fishrhessianacc}: yet, \enquote{Hessian is an order of magnitude more computationally intensive} than individual gradients (see Fig.\ 9 in \citet{dangel2020backpack}) and is not yet practical directly as a training objective.

In conclusion, we \textit{first} compute the individual derivatives of ERM in $w_{\omega}$ using BackPACK to get $\{\operatorname{Diag}(\mC_e)\}_{e\in \mathcal{E}}$ and \textit{second} backpropagate the loss from Eq.\ \ref{eq:loss} in the whole network (without keeping the individual gradients). Fishr is simple to implement (see the pseudo-code in Appendix \ref{appendix:pseudocode}) and at low computational costs. For example, on PACS dataset (7 classes and $|\omega|=14,343$) with a ResNet-50 and batch size 32, Fishr induces an overhead in memory of +0.2\% and in training time of +2.7\% (with a Tesla V100) compared to ERM; on the larger-scale DomainNet (345 classes and $|\omega|=706,905$), the overhead is +7.0\% in memory and +6.5\% in training time. As a side note, keeping the full covariance of size $|\omega|^2\approx5\times10^8$ on DomainNet would not have been possible.%

% PACS

% 10609MiB and 0.5219788551
% 10631 and 0.5337302216
% DomainNet:
% erm: 17511MiB/17513MiB
% 0.5606605053
% fishr: 19339MiB/19341MiB
% 0.5810389996
% sum([np.prod(p.size()) for p in filter(lambda p: p.requires_grad, self.featurizer.parameters())])
% 23_508_032
% 706905*6

% PACS
% 11180/11158
% 0.3475346565246582/0.3385164737701416
% ERM: 8.189440727233887, 0.3377034664154053
% Fishr: 8.19534683227539, 0.3475346565246582
% Net
% 18736/17516
% 0.5951297283172607/0.5586967468261719
% 13.406212329864502/15.247553825378418
% ERM: 13.136273860931396, 0.5860002040863037
% ERM: 17514
% Fishr: 14.979307651519775, 0.6448450088500977
% Fishr: 18732


==> sections/model/backup/03_1_model_iclr.tex <==
\subsection{Fishr matches the domain-level gradient distributions}
\label{model:fishrmatchgradient}

The first motivation for Fishr is the independence between the gradient and the domain random variables.
This is achieved by matching the diagonals of the covariance of the empirical gradient distributions $\left\{\vg_{e}^{i}\right\}_{i=1}^{n_e}$ across training domains $e \in \mathcal{E}$.
Indeed, this is an efficient and well-suited method to align distributions.
This was recently highlighted by the success of the covariance-based CORAL \citep{coral216aaai} on the DomainBed benchmark: matching covariance performed better than adversarial methods to align feature distributions.
Therefore, this motivates the use of gradient variance: more complex strategies to align gradient distributions are best left for future works.


We now provide three reasons to enforce distributional invariance in gradients rather than in features.
% \begin{enumerate}
% \textit{First and foremost}, having similar domain-level gradient distributions is critical so that the DNN has shared properties across domains. Indeed, gradient disagreements and pairwise relations dictate the optimization of DNNs \citep{faghri2020study}: for instance, gradient confusion slows down convergence \citep{sankararaman2020impact} even though gradient diversity improves generalization \citep{yin2018gradient}. The gradient mean alone can not capture these statistics.
% % These statistics can not be captured by only the gradient mean.
% \textit{Second}, gradients are more expressive and richer than features. Specifically, gradients were shown to better cluster semantically close inputs \citep{fort2019stiffness,He2020The}.
% When comparing the features extracted for two inputs \citep{johnson2016perceptual}, a small difference in activation may be multiplied by large subsequent weights and lead to distant predictions.
% On the contrary when comparing gradients, each activation is weighted by its true importance for the prediction \citep{charpiat2019input}.
% % Notably, as stated in Theorem 1 in \citet{charpiat2019input}, similar gradients imply similar features.
% % A small difference in features could be counterbalanced by a relatively high following parameters, leading to high differences in predictions.
% %On the contrary, gradients take into account the relative importance of weights by considering activation in line with the potential impact on their output on the final loss.
% \textit{Third}, gradient includes the label $Y$ in its expression. Hence, gradient-based approaches are `label-aware' by design. In contrast, most feature-based methods fail in case of label shift, \textit{i.e.}, when $P(Y|E) \neq P(Y)$ \citep{zhao2019learning,johansson2019support}.
% %could potentially detect distribution input shifts ($P(X|E) \neq P(X)$) but
% % that rely on strict assignations.
% % and would not be directly applicable with multi-labels or in regression.
% % similar gradients variance is critical to align generalization abilities across domains - .
% %yet they are left to show any improvements for OOD generalization \citep{gulrajani2021in} when not computationally unfeasible on large scale data \citep{pmlr-v28-zhang13d}.
% % Previous class-conditional features-based approaches have been developed, by matching the conditional distributions $P(Z|Y, E)$ and $P(Z|Y)$ \citep{li2018domaincond,pmlr-v48-gong16} or with importance sampling \citep{lipton2018detecting,azizzadenesheli2018regularized,NEURIPS2020_dfbfa7dd}, yet they are left to show any improvements for OOD generalization \citep{gulrajani2021in} when not computationally unfeasible on large scale data \citep{pmlr-v28-zhang13d}.
% % On the contrary, our gradients-based approach is label-aware by design as the loss includes $Y$.
% \textit{Lastly}, matching gradient also matches training risks, as motivated in V-REx \citep{krueger2020utofdistribution} to improve OOD generalization. Indeed, gradient amplitudes are directly weighted by the loss values. This is empirically validated in Appendix \ref{appendix:fishrrex}, where we show that Fishr induces $|\mathcal{R}_{A} - \mathcal{R}_{B}|^2 \to 0$ when $\mathcal{E}=\{A, B\}$.
% \end{enumerate}
% \begin{enumerate}
%     \item Having similar domain-level gradient distributions is critical so that the DNN has shared properties across domains. Indeed, gradient disagreements and pairwise relations are key to the optimization procedure of DNNs: for instance, gradient confusion slows down convergence \citep{sankararaman2020impact} even though gradient diversity improves generalization \citep{yin2018gradient}. The gradient mean can capture the average learning direction but can not capture these refined statistics.
%           % These statistics can not be captured by only the gradient mean.
%     \item Gradients are more expressive and richer than features. Specifically, gradients were shown to better cluster semantically close inputs \citep{fort2019stiffness,He2020The}.
%           When comparing the features extracted for two inputs \citep{johnson2016perceptual}, a small difference in activation may be multiplied by large subsequent weights and lead to distant predictions.
%           On the contrary when comparing gradients, each activation is weighted by its true importance for the prediction \citep{charpiat2019input}.
%           % Notably, as stated in Theorem 1 in \citet{charpiat2019input}, similar gradients imply similar features.
%           % A small difference in features could be counterbalanced by a relatively high following parameters, leading to high differences in predictions.
%           %On the contrary, gradients take into account the relative importance of weights by considering activation in line with the potential impact on their output on the final loss.
%     \item Gradients take into account the label $Y$, which appears as an argument for the loss $\ell$. Hence, gradient-based approaches are `label-aware' by design. In contrast, seminal feature-based methods were shown to fail in case of label shift, \textit{i.e.}, when $P(Y|E) \neq P(Y)$, because they do not consider $Y$ \citep{zhao2019learning,johansson2019support}.
%           %could potentially detect distribution input shifts ($P(X|E) \neq P(X)$) but
%           % that rely on strict assignations.
%           % and would not be directly applicable with multi-labels or in regression.
%           % similar gradients variance is critical to align generalization abilities across domains - .
%           %yet they are left to show any improvements for OOD generalization \citep{gulrajani2021in} when not computationally unfeasible on large scale data \citep{pmlr-v28-zhang13d}.
%           % Previous class-conditional features-based approaches have been developed, by matching the conditional distributions $P(Z|Y, E)$ and $P(Z|Y)$ \citep{li2018domaincond,pmlr-v48-gong16} or with importance sampling \citep{lipton2018detecting,azizzadenesheli2018regularized,NEURIPS2020_dfbfa7dd}, yet they are left to show any improvements for OOD generalization \citep{gulrajani2021in} when not computationally unfeasible on large scale data \citep{pmlr-v28-zhang13d}.
%           % On the contrary, our gradients-based approach is label-aware by design as the loss includes $Y$.
%     \item Matching gradient distributions also matches training risks, as motivated in V-REx \citep{krueger2020utofdistribution} to improve OOD generalization. Indeed, gradient amplitudes are directly weighted by the loss values. This is empirically validated in Appendix \ref{appendix:fishrrex}, where we show that Fishr induces $|\mathcal{R}_{A} - \mathcal{R}_{B}|^2 \to 0$ when $\mathcal{E}=\{A, B\}$.
% \end{enumerate}
% \textit{First and foremost}, having similar domain-level gradient distributions is critical so that the DNN has shared properties across domains. Indeed, gradient disagreements and pairwise relations are key to the optimization procedure of DNNs: for instance, gradient confusion slows down convergence \citep{sankararaman2020impact} even though gradient diversity improves generalization \citep{yin2018gradient}. The gradient mean can capture the average learning direction but can not capture these refined statistics. As a side note,
% Moreover, gradients are more expressive and richer than features. Specifically, gradients were shown to better cluster semantically close inputs \citep{fort2019stiffness,He2020The}.
% When comparing the features extracted for two inputs \citep{johnson2016perceptual}, a small difference in activation may be multiplied by large subsequent weights and lead to distant predictions.
% On the contrary when comparing gradients, each activation is weighted by its true importance for the prediction \citep{charpiat2019input}.
\textit{Second}, gradients take into account the label $Y$, which appears as an argument for the loss $\ell$. Hence, gradient-based approaches are `label-aware' by design. In contrast, seminal feature-based methods were shown to fail in case of label shifts, because they do not consider $Y$ \citep{johansson2019support,zhao2019learning}.
Gradients were shown to efficiently cluster semantically close inputs \citep{fort2019stiffness,He2020The,charpiat2019input} and to be more expressive and richer than features.
\textit{Lastly}, matching gradient distributions also matches training risks, as motivated in V-REx \citep{krueger2020utofdistribution}. Indeed, gradient amplitudes are directly weighted by the loss values. This is theoretically proved in Appendix \ref{appendix:lineartheory}, and empirically validated in Appendix \ref{appendix:fishrrex}: Fishr induces $|\mathcal{R}_{A} - \mathcal{R}_{B}|^2 \to 0$ when $\mathcal{E}=\{A, B\}$ for Colored MNIST.
% Nonetheless, it is worth noting that the main drawback of using gradients is the computational overhead: this will be tackled in Section \ref{model:implem}.



==> sections/model/backup/03_2_model_iclr.tex <==
\subsection{Theoretical Analysis: Fishr reduces inconsistencies across the domain-level loss landscapes}
\label{model:fishrmatchloss}

In Section \ref{model:covfimhe}, we argue (based on previous works) and show (in Table \ref{table:hessianermfishr}) that Fishr matches the domain-level Hessians.
The gradient covariance, computable efficiently with a unique backpropagation, serves as a proxy for the Hessian. Thus, we use the second moment of the first-order derivatives to regularize the second-order derivatives.
Then, we justify in Section \ref{model:whyhessian} why similar domain-level Hessians reduces inconsistencies in the loss landscape and improves generalization.

\subsubsection{Fishr matches the domain-level Hessians}
\label{model:covfimhe}

The Hessian matrix $\mH=\sum_{i=1}^{n} \nabla_{\theta}^{2} \ell\left(f_{\theta}(\vx^i), \vy^{i}\right)$ captures the second-order derivatives of the objective and is of key importance for deep learning methods. Yet, $\mH$ is computationally demanding and can not be computed directly in general. Recent methods \citep{izmailov2018averaging,foret2021sharpnessaware} tackle the Hessian indirectly by modifying the learning procedure. In contrast, we use the fact that the Fisher Information Matrix $\mF=\sum_{i=1}^{n} \E_{\hat{\vy} \sim P_{\theta}(\cdot|\vx^i)} \left[ \nabla_{\theta} \log p_{\theta}(\hat{\vy}|\vx^i) \nabla_{\theta} \log p_{\theta}(\hat{\vy}|\vx^i)^{\top}\right]$ \citep{fisher1922mathematical,raofim1945} approximates $\mH$, with theoretically probably bounded errors under mild assumptions \citep{schraudolph2002fast}.
Yet, $\mF$ remains costly as it demands one backpropagation per class. That's why most empirical works (\textit{e.g.}, in compression \citep{frantar2021fficient,pmlr-v139-liu21ab} and optimization \citep{dangel2021vivit}) approximate $\mH$ with
the `empirical' Fisher Information Matrix $\tilde{\mF}=\mG_{e}^{\top} \mG_{e}=\sum_{i=1}^{n}\nabla_{\theta} \log p_{\theta}(\vy^i|\vx^i)\nabla_{\theta}\log p_{\theta}(\vy^i|\vx^i)^{\top}$ \citep{martens2014new} where $p_{\theta}(\cdot|\vx)$ is the density predicted by $f_{\theta}$ on input $\vx$.
While $\mF$ uses the model distribution $P_{\theta}(\cdot|X)$, $\tilde{\mF}$ uses the data distribution $P(Y|X)$.
Despite this key difference, $\tilde{\mF}$ and $\mF$ were shown to share the same structure and to be similar up to a scalar factor \citep{interplayinfomatrix2020}.
This was discussed in \citet{li2020hessian} and further highlighted even at early stages of training (before overfitting) in the Fig.\ 1 and the Appendix S3 of \citet{NEURIPS2020_d1ff1ec8}.

% \input{tables/irm/cmnist_hessian.tex}
\begin{table}[h]
    % \vspace{-2.em}
    \centering
    \caption{
        \textbf{Invariance analysis at convergence in Colored MNIST} across the two training domains $\mathcal{E}=\{90\%,80\%\}$. Details in Section \ref{expe:irmcmnist}.
        Compared to ERM, Fishr matches the gradient variance ($\operatorname{Diag}(\mC_{90\%})\approx\operatorname{Diag}(\mC_{80\%})$).
        Most importantly, this enforces invariance in domain-level risks ($\mathcal{R}_{90\%}\approx\mathcal{R}_{80\%}$) (as further shown in Appendix \ref{appendix:fishrrex}) and in domain-level Hessians ($\operatorname{Diag}(\mH_{90\%})\approx\operatorname{Diag}(\mH_{80\%})$) (as further shown in Fig.\ \ref{fig:fishrhessianacc} and in Appendix \ref{appendix:hessianmatching}).
    }
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{c c c}
            \toprule
                                                                                           & ERM                  & Fishr                \\
            \midrule
            $\left\|\Var(\mG_{90\%})-\Var(\mG_{80\%})\right\|_{F}^{2}$ & $3.1 \times 10^{-3}$ & $2.2 \times 10^{-6}$ \\
            $\left\|\mathcal{R}_{90\%} - \mathcal{R}_{80\%}\right\|_{2}^{2}$               & $1.1 \times 10^{-2}$ & $4.2 \times 10^{-7}$ \\
            % \midrule
            $\left\|\operatorname{Diag}\left(\mH_{90\%}-\mH_{80\%}\right)\right\|_{F}^{2}$ & $2.6 \times 10^{-4}$ & $2.0 \times 10^{-6}$ \\
            \bottomrule%
        \end{tabular}%
    }%
    \label{table:hessianermfishr}%
\end{table}%%
% erm vrex 0.010677835624665021
% fishr: vrex 4.170017291471595e-07


Critically, $\tilde{\mF}$ is nothing else than the unnormalized uncentered covariance matrix when $\ell$ is the negative log-likelihood. Thus, $\mC$ and $\tilde{\mF}$ are equivalent (up to the multiplicative constant $n$) at any first-order stationary point: so $\mC \approxprop \tilde{\mF}$. Overall, this suggests that $\mC$ and $\mH$ are closely related.
In our multi-domain framework, we define the domain-level matrices with the subscript $e$.
Table \ref{table:hessianermfishr} empirically confirms that matching $\{\operatorname{Diag}(\mC_e)\}_{e\in\mathcal{E}}$  --- i.e., $\{\Var(\mG_e)\}_{e\in\mathcal{E}}$  --- with Fishr forces the domain-level Hessians $\{\operatorname{Diag}(\mH_e)\}_{e\in\mathcal{E}}$ to be aligned at convergence (in the classifier $w_{\omega}$ for computational reasons).

Even so, we acknowledge that approximating $\mH$ by $\tilde{\mF}$ is not fully justified theoretically \citep{martens2014new,NEURIPS2019_46a558d9}.
One would hope that when overfitting occurs, $P_{\theta}(\cdot|X) \to P(Y|X)$ and then $\mF \to \tilde{\mF}$. Though, this requires strong assumptions such as $\chi^2$ convergence (see Proposition 1 in \citet{interplayinfomatrix2020}).
% Yet, the issues with $\mF$ are that $\mF$ ignores the label $Y$ and that its computation demands additional backpropagations.
% % However, computing $\mF$ ignores the label $Y$ and demands additional backpropagations.
% Thus, notably for computational efficiency, we consider $\tilde{\mF}$ (and by extension $\mC$) and not $\mF$.
% % to trade off theoretical guarantees
% Yet, using domain-level $\{\mF_e\}_{e\in\mathcal{E}}$ ignores the label $Y$ and : this is best left for future work.
In this paper, we trade off theoretical guarantees for computational efficiency and consider $\mC$ and $\tilde{\mF}$.
Notably, Appendix \ref{appendix:centered} shows that matching the diagonals of $\{\mC_e\}_{e\in\mathcal{E}}$ or $\{\tilde{\mF}_e\}_{e\in\mathcal{E}}$ --- \textit{i.e.}, centering or not the statistics --- perform similarly.
% Yet, the issues with $\mF$ are that $\mF$ ignores the label $Y$ and that its computation demands additional backpropagations.
% % However, computing $\mF$ ignores the label $Y$ and demands additional backpropagations.
% Thus, notably for computational efficiency, we consider $\tilde{\mF}$ (and by extension $\mC$) and not $\mF$.


\subsubsection{Invariant Hessians for loss consistency}
\label{model:whyhessian}
\input{pictures/model/fig_consistency.tex}
To understand why having similar domain-level Hessians at convergence improves generalization, we leverage the \textbf{inconsistency} formalism developed in AND-mask \citep{parascandolo2021learning}.
They argue that \enquote{patchwork solutions sewing together different strategies} for different domains may not generalize well: good weights should be optimal on all domains and \enquote{hard to vary} \citep{hardtovary}.
% Intuitively, averaging across domains destroy information critical.
They formalize this intuition with an inconsistency score \linebreak
$\mathcal{I}^{\epsilon}\left(\theta^{*}\right)=\max_{(A, B)\in\mathcal{E}^2} \max_{\theta \in N_{A, \theta^{*}}^{\epsilon}}\left|\mathcal{R}_{B}(\theta)-\mathcal{R}_{A}(\theta^{*})\right|$ where
$\theta \in N_{A, \theta^{*}}^{\epsilon}$ if there is a path in the weights space between $\theta$ and $\theta^{*}$ where the risk $\mathcal{R}_{A}$ remains in an $\epsilon>0$ interval around $\mathcal{R}_{A}(\theta^{*})$.
$\mathcal{I}$ increases with conflicting geometries in the loss landscapes around $\theta^{*}$ as in Fig.\ \ref{fig:fig_consistenty}: \textit{i.e.}, when another `close' solution $\theta$ is equivalent to the current solution $\theta^{*}$ in a domain $A$ but yields different losses in $B$.


% in the weights space
% $\mathcal{A}=\left\{A,B\right\}$ and
Moreover, the Hessian approximates the local curvature of the loss landscape around $\theta^{*}$.
Using this fact and a second-order Taylor expansion of the loss, we derive in Appendix \ref{appendix:hardtovary} a new upper bound of domain inconsistencies.
Assuming that domain-level Hessians are co-diagonalizable for simplicity, inconsistency increases when an eigenvalue is small in $\mH_A$ but large in $\mH_B$: indeed, a small weight perturbation in the direction of the associated eigenvector would change the loss slightly in the domain $A$ but drastically in $B$.
In conclusion, \enquote{inconsistency is lowest when shapes \textelp{} are similar} \citep{parascandolo2021learning}, \textit{i.e.}, when $\mH_A=\mH_B$.
AND-mask minimizes $\mathcal{I}$ by zeroing out gradients with inconsistent directions across domains. However, this masking strategy introduces dead zones \citep{shahtalebi2021andmask} in weights where the model could get stuck, ignores gradient magnitudes and empirically performs poorly with `real' datasets from DomainBed.
In place, \textbf{Fishr reduces inconsistencies in the loss landscapes across domains by matching the domain-level Hessians}, using domain-level gradient variances as a proxy.

Finally, we refer the readers to Appendix \ref{appendix:ntk} where we leverage the Neural Tangent Kernel (NTK) \citep{NEURIPS2018_5a4be1fa} theory to further motivate the gradient variance matching during the optimization process --- and not only at convergence. In brief, as $\mF$ and the NTK matrices share the same non-zero eigenvalues, similar $\{\mC_e\}_{e\in\mathcal{E}}$ during training reduce the simplicity bias by preventing the learning of different domain-dependent shortcuts at different training speeds: this favors a shared mechanism that predicts the same thing for the same reasons across domains.
% explanations


==> tables/bias-mitigators/bmnist.tex <==
% \begin{table}[!h]%
% \caption{\textbf{BMnist dataset}.}
% \centering
% \resizebox{0.80\textwidth}{!}{%
% \begin{tabular}{lccccc}
%     \hline Groups/,\multicolumn{2}{c} { Male } & \multicolumn{2}{c} { Non-Male } & Unbiased \\
%     Methods & NonBlond & Blond & NonBlond & Blond & Accuracy \\
%     \hline
%     % --lr 1e-3 --weight_decay 0
%     ERM &  99.5 & 35.5 & 95.9 & 82.8 & 78.4 \\
%     \hline
%     \hline
% \end{tabular}%
% }
% \label{table:bmnist}%
% \end{table}


% strategy
% * 0
% 50 => 68
% * 1
% 51 => 60
% * 2
% 47=>57
% * 3
% 43=>53
% * 4
% 46=>56


==> tables/bias-mitigators/celeba.tex <==
\begin{table}[!h]%
\caption{\textbf{CelebA dataset}.}%
\centering%
\resizebox{0.80\textwidth}{!}{%
\begin{tabular}{cccccc}%
\toprule
& \multicolumn{2}{c} { Male } & \multicolumn{2}{c} { Non-Male } & \textbf{Unbiased} \\
Methods & NonBlond & Blond & NonBlond & Blond & \textbf{Accuracy} \\
\hline
ERM & 99.3 & 42.8 & 95.9 & 83.3 & 80.3\\
Up Wt & 89.3 & 77.8 & 87.4 & 95.0 & 87.4 \\
GDRO & 91.2 & 80.0 & 90.9 & 92.1 & 88.5 \\
RUBi & 96.6 & 68.9 & 94.3 & 89.1 & 87.2 \\
LNL & 99.1 & 39.4 & 95.4 & 82.8 & 79.2 \\
IRM & 99.1 & 40.6 & 95.9 & 83.6 & 79.8 \\
LFF & 96.0 & 46.1 & 90.4 & 80.0 & 77.8 \\
SD & 96.4 & 73.3 & 88.0 & 96.6 & 88.6 \\
% \hline
% --lr 1e-3 --weight_decay 0
% ERM &  99.5 & 35.5 & 95.9 & 82.8 & 78.4 \\
\midrule
% % --lr 1e-3 --grad_penalty_weight 1 --weight_decay 0
% Fisheral 20 & 93.3 & 81.7 & 91.7 & 89.24 & 88.9 \\
% Fisheral 30 & 94.7 & 74.4 & 90.5 & 91.2 & 87.7 \\
% Fisheral 40 & 98.5 & 43.8 & 96.5 & 77.9 & 79.0 \\
% Fisheral 50 & 97.0 & 53.8 & 91.9 & 90.2 & 83.2 \\
% --lr 1e-3 --grad_penalty_weight 2 --weight_decay 0
% Fisheral 44 & 72.6 & 78.3 & 81.3 & 88.18 & 80 \\
% --lr 1e-4 --grad_penalty_weight 1 --weight_decay 0
% Fisheral 20 & 86.55 & 83.33 & 87.26 & 92.94 & 87.5 \\
% Fisheral 50 & 86.7 & 90 & 81.8 & 96.5 & 88.7 \\
% --expt_type celebA_experiments --trainer_name FisheralTrainer --lr 1e-4 --grad_penalty_weight 1.0 --weight_decay 0 --root_dir /net/big/rame//dataplace/ --strategy 0 --num_envs_per_batch 4
% Fisheral$^{*}$ & 92.0 & 81.6 & 88.3 & 94.3 & 89.1 \\
% % --lr 1e-5 --grad_penalty_weight 1.0 --weight_decay 0 --root_dir /net/big/rame//dataplace/ --strategy 2 --num_envs_per_batch 4
% Fisheral & 90.2 & \textbf{87.7} & 90.2 & 94.5 & \textbf{90.5} \\
% % grad_penalty_weight 0.5
% Fisheral 50 & 91.7 & 80.5 & 85.8 & 95.4 & 88.2 \\
% % grad_penalty_weight 1.5
% Fisheral 50 & 92.5 & 78.9 86.15 & 94.9 & 87.1 \\
% % grad_penalty_weight 2
% Fisheral 50 & 83.7 & 87.2 & 79.3 & 98.0 & 87.1 \\
% % --lr 1e-4 --grad_penalty_weight 1 --weight_decay 0 -penalty_anneal_iters 10
% Fisheral 50 & 96.8 & 65 & 91.5 & 90.5 & 85.7 \\
% % -penalty_anneal_iters 10
% Fisheral 50 & 79.5 & 87.8 & 68.7 & 98.5 & 85.7 \\
% % lr 1e-5 --grad_penalty_weight 1
% Fisheral 50 & 81.2 & 83.9 & 84.3 & 92.7 & 85.8
% --lr 1e-4 --grad_penalty_weight 1.0 --weight_decay 0 --strategy 1
% Fisheral & 92.4 & 80.5 & 89.2 & 94.0 & 89.1 \\
% --strategy 3
% Fisheral 3 & 80.0 & 80.5 & 71.2 & 95.7 & 82.05 \\
% % --strategy 5
% Fisheral 5 & 99.0 & 29.5 & 96.2 & 80.7 & 76.2 \\
% strategy 2: smaller leanring rate
% \midrule
% --trainer_name FisheralTrainer --lr 1e-5 --grad_penalty_weight 0.1 --weight_decay 0 --root_dir /net/big/rame//dataplace/ --strategy 4
% Fisheral Biaspairs & 90.9 & 81.7 & 91.2 & 92.0 & 89.0 \\
% Fisheral Biaspairs & 90.7 & 86.6 & 90.8 & 92.4 & 90.1 \\ % step 49
% --lr 1e-5 --grad_penalty_weight 0.2 --weight_decay 0 --root_dir /net/big/rame//dataplace/ --strategy 4 --num_envs_per_batch 4
% Fisheral Biaspairs & 91.3 & 82.8 & 90.9 & 92.2 & 89.3 \\
% --lr 1e-5 --grad_penalty_weight 1 --weight_decay 0 --root_dir /net/big/rame//dataplace/ --strategy 4 --num_envs_per_batch 4
% Fisheral Biaspairs & 90.5 & 81.1 & 90.1 & 91.9 & 88.4 \\
% --lr 1e-5 --grad_penalty_weight 0.01 --strategy 4
% --lr 1e-5 --grad_penalty_weight 10 --strategy 14
% Fisheral & 90.2 & \textbf{88.3} & 89.9 & 93.5 & \textbf{90.5} \\
% Fisheral & 89.2 & \textbf{90.0} & 89.1 & 94.2 & \textbf{90.5} \\
% --lr 1e-5 --grad_penalty_weight 50. --strategy 14
% Fisheral & 91.8 & \textbf{86.7} & 91.3 & 92.2 & \textbf{90.5} \\
% --lr 1e-5 --grad_penalty_weight 0.01 --strategy 4 --weight_decay 1e-5
% Fisheral & 89.1 & \textbf{90.0} & 89.1 & 93.9 & \textbf{90.5} \\
% --lr 1e-5 --grad_penalty_weight 10 --strategy 14 --weight_decay 1e-5
% Fisheral & 89.4 & 90.0 & 89.0 & 94.5 & 90.7 \\
% --lr 1e-5 --grad_penalty_weight 50. --strategy 14 --weight_decay 1e-5
% Fisheral & 91.4 & 86.1 & 90.6 & 92.2 & 90.2 \\
% /net/big/rame/dataplace/Bias-Mitigators/CelebA/predict_Blond_Hair/FisheralTrainer/lr_1e-05_wd_1e-05-2107061030-14-50.0
% CUDA_VISIBLE_DEVICES=1 python main.py --expt_type celebA_experiments --trainer_name FisheralTrainer --lr 1e-5 --grad_penalty_weight 50 --strategy 14 --weight_decay 1e-5
% FisherAl & 91.2 & 88.9 & 90.0 & 93.8 & \textbf{91.0} \\
% \midrule
% --lr 1e-5 --grad_penalty_weight 1.0 --weight_decay 0 --root_dir /net/big/rame//dataplace/ --strategy 6
% FisheralCond & 90 & 82.2 & 90.5 & 91.6 & 88.6 \\ % galere à overfitter mais très bon
% FisheralCond & 90.5 & 83.3 & 90.1 & 93.0 & 89.3 \\ % 0.01 ?
% %  --lr 1e-4 --grad_penalty_weight 1.0 --weight_decay 0 --root_dir /net/big/rame//dataplace/ --strategy 7
% FisheralCond & 91.5 & 81.1 & 89.5 & 94.9 & 89.3 \\
% FisheralCond & 92.1 & 82.2 & 91.2 & 91.8 & 89.3 \\ % 1e-5 and 0.05
% FisheralCond & 89.6 & 87.8 & 89.0 & 94.2 & 90.2 \\ % 1e-5 and 0.01 --strategy 6
% CUDA_VISIBLE_DEVICES=2 python main.py --expt_type celebA_experiments --trainer_name FisheralTrainer --lr 1e-5 --grad_penalty_weight 10. --strategy 16
% FisherAlCond & 89.5 & 90.6 & 89.2 & 94.1 & 90.8 \\
% FisherAlCond & 89.5 & 90.6 & 89.2 & 94.1 & 90.8 \\
% \midrule
% % conditional with shared ema
% % --lr 1e-5 --grad_penalty_weight 1.0 --strategy 8
% % FisheralCond & 88.5 & 85.5 & 88.8 & 93.0 & 88.9 \\
% FisheralCond & 88.5 & 86.6 & 88.5 & 94.6 & 89.6 \\ % 1
% % --lr 1e-5 --grad_penalty_weight 0.1 --strategy 8
% FisheralCond & 91.5 & 84.0 & 91.0 & 94.6 & 89.7 \\ % 0.1
% /net/big/rame/dataplace/Bias-Mitigators/CelebA/predict_Blond_Hair/FisheralTrainer/lr_1e-05_wd_1e-05-2107140918-142-20.0
% FisherMat & 89.9 & 87.8 & 89.6 & 93.9 & \textbf{90.3} \\
% CUDA_VISIBLE_DEVICES=2 python main.py --expt_type celebA_experiments --trainer_name FisheralTrainer --lr 1e-5 --grad_penalty_weight 100 --strategy 142 --weight_decay 1e-4
FisherMat & 91.5 & 85.6 & 90.7 & 93.0 & \textbf{90.2} \\
\bottomrule
\end{tabular}}%
\label{table:celeba}%
\end{table}%
% 66.0,35.0,70.5,34.5,41.2,37.8,68.1,34.8,68.3,34.9,64.5,35.1,65.6,35.0
% % 38, 40.9, 38.1, 38.3, 39.7, 37.5, 38.5
% 86.55,83.33,87.26,92.94
% 72.6,78.3,81.3,88.18


==> tables/domainbed/archi.tex <==

\begin{table}[h]
    \caption{Neural network architectures used for each dataset.}
    \centering
    \begin{tabular}{ll}
        \toprule
        \textbf{Dataset} & \textbf{Architecture}          \\
        \midrule
        Colored MNIST /  & \multirow{2}{*}{MNIST ConvNet} \\
        Rotated MNIST    &                                \\
        \midrule
        VLCS / PACS /    & \multirow{4}{*}{ResNet-50}     \\
        OfficeHome /     &                                \\
        TerraIncognita / &                                \\
        DomainNet        &                                \\
        \bottomrule
    \end{tabular}
    \label{table:archi}
\end{table}%

% \begin{table}{}
%     \caption{MNIST ConvNet architecture.}
%     \centering
%     \begin{tabular}{ll}
%         \toprule
%         \textbf{\#} & \textbf{Layer}                                     \\
%         \midrule
%         1           & Conv2D $(\mathrm{in}=d$, out $=64)$                \\
%         2           & ReLU                                               \\
%         3           & GroupNorm (groups $=8)$                            \\
%         4           & Conv2D $(\mathrm{in}=64$, out $=128$, stride $=2)$ \\
%         5           & ReLU                                               \\
%         6           & GroupNorm (8 groups)                               \\
%         7           & Conv2D (in=128, out=128)                           \\
%         8           & ReLU                                               \\
%         9           & GroupNorm (8 groups)                               \\
%         10          & Conv2D (in=128, out=128)                           \\
%         11          & ReLU                                               \\
%         12          & GroupNorm (8 groups)                               \\
%         13          & Global average-pooling                             \\
%         \bottomrule
%     \end{tabular}
%     \label{table:mnistconvnet}
% \end{table}



==> tables/domainbed/table_iga_warmup.tex <==
\begin{table}[ht]%
    \caption{\textbf{Fishr (gradient covariance) vs.\ IGA (gradient mean)} on DomainBed's Colored MNIST.}%
    \centering
    \adjustbox{width=0.75\textwidth}{
        \begin{tabular}{llllcccccccc}
            \toprule
            \textbf{Model selection}  & \textbf{Algorithm}     & \textbf{Gradients in}      & \textbf{Warmup} & \textbf{ema} & \textbf{+90\%}          & \textbf{+80\%}          & \textbf{10\%}           & \textbf{Avg}  \\
            \midrule
            \midrule
            \multirow{8}{*}{Oracle}   & ERM                    & N/A                        & N/A             & N/A          & 71.8 $\pm$ 0.4          & 72.9 $\pm$ 0.1          & 28.7 $\pm$ 0.5          & 57.8          \\
            \cmidrule{2-9}
                                      & \multirow{4}{*}{IGA}   & $\theta=(\phi, \omega)$    & \xmark          & \xmark       & 71.8 $\pm$ 0.5          & 73.0 $\pm$ 0.3          & 29.2 $\pm$ 0.5          & 58.0          \\
                                      &                        & $\omega$                   & \xmark          & \xmark       & 72.4 $\pm$ 0.1          & \textbf{73.3} $\pm$ 0.2 & 29.3 $\pm$ 0.6          & 58.3          \\
                                      &                        & $\omega$                   & \cmark          & \xmark       & 72.5 $\pm$ 0.2          & \textbf{73.3} $\pm$ 0.1 & 31.8 $\pm$ 0.7          & 59.2          \\
                                      &                        & $\omega$                   & \cmark          & \cmark       & 72.6 $\pm$ 0.3          & 72.9 $\pm$ 0.2          & 50.0 $\pm$ 1.2          & 65.2          \\
            \cmidrule{2-9}
                                      & \multirow{3}{*}{Fishr} & \multirow{3}{*}{ $\omega$} & \xmark          & \xmark       & 73.0 $\pm$ 0.3          & 73.2 $\pm$ 0.1          & 29.5 $\pm$ 1.1          & 58.6          \\
                                      &                        &                            & \cmark          & \xmark       & 72.7 $\pm$ 0.3          & 72.8 $\pm$ 0.1          & 34.0 $\pm$ 4.5          & 59.8          \\
                                      &                        &                            & \cmark          & \cmark       & \textbf{74.1} $\pm$ 0.6 & \textbf{73.3} $\pm$ 0.1 & \textbf{58.9} $\pm$ 3.7 & \textbf{68.8} \\
            \midrule
            \multirow{8}{*}{Training} & ERM                    & N/A                        & N/A             & N/A          & 71.7 $\pm$ 0.1          & 72.9 $\pm$ 0.2          & 10.0 $\pm$ 0.1          & 51.5          \\
            \cmidrule{2-9}
                                      & \multirow{4}{*}{IGA}   & $\theta=(\phi, \omega)$    & \xmark          & \xmark       & 71.8 $\pm$ 0.3          & 73.2 $\pm$ 0.2          & 9.8 $\pm$ 0.0           & 51.6          \\
                                      &                        & $\omega$                   & \xmark          & \xmark       & 71.8 $\pm$ 0.1          & 73.2 $\pm$ 0.2          & \textbf{10.1} $\pm$ 0.0 & 51.7          \\
                                      &                        & $\omega$                   & \cmark          & \xmark       & 71.8 $\pm$ 0.2          & 73.1 $\pm$ 0.2          & \textbf{10.1} $\pm$ 0.0 & 51.7          \\
                                      &                        & $\omega$                   & \cmark          & \cmark       & \textbf{72.5} $\pm$ 0.4 & 73.3 $\pm$ 0.2          & \textbf{10.1} $\pm$ 0.1 & \textbf{52.0} \\
            \cmidrule{2-9}
            %   & Fishr                  & $\omega$                    & \cmark       & 72.3 $\pm$ 0.9          & \textbf{73.5} $\pm$ 0.2 & \textbf{10.1} $\pm$ 0.2 & \textbf{52.0} \\
                                      & \multirow{3}{*}{Fishr} & \multirow{3}{*}{$\omega$}  & \xmark          & \xmark       & 71.6 $\pm$ 0.1          & 73.2 $\pm$ 0.1          & 9.9 $\pm$ 0.0           & 51.6          \\
                                      &                        &                            & \cmark          & \xmark       & 71.1 $\pm$ 0.6          & \textbf{73.6} $\pm$ 0.1 & \textbf{10.1} $\pm$ 0.2 & 51.6          \\
                                      &                        &                            & \cmark          & \cmark       & 72.3 $\pm$ 0.9          & 73.5 $\pm$ 0.2          & \textbf{10.1} $\pm$ 0.2 & \textbf{52.0} \\
            \bottomrule
        \end{tabular}
    }
    \label{table:igacmnist}
\end{table}

\begin{table}[ht]%
    \caption{\textbf{Fishr (gradient covariance) vs.\ IGA (gradient mean)} on DomainBed's OfficeHome.}%
    \centering
    \adjustbox{width=0.85\textwidth}{
        \begin{tabular}{llllcccccccc}
            \toprule
            \textbf{Model selection}  & \textbf{Algorithm}     & \textbf{Gradients in}     & \textbf{Warmup} & \textbf{ema} & \textbf{A}              & \textbf{C}              & \textbf{P}              & \textbf{R}              & \textbf{Avg}  \\
            \midrule
            \midrule
            \multirow{8}{*}{Oracle}   & ERM                    & N/A                       & N/A             & N/A          & 61.7 $\pm$ 0.7          & 53.4 $\pm$ 0.3          & 74.1 $\pm$ 0.4          & 76.2 $\pm$ 0.6          & 66.4          \\
            \cmidrule{2-10}
                                      & \multirow{4}{*}{IGA}   & $\theta=(\phi, \omega)$   & \xmark          & \xmark       & 50.1 $\pm$ 2.5          & 49.6 $\pm$ 1.6          & 59.5 $\pm$ 6.7          & 68.5 $\pm$ 1.2          & 56.9          \\
                                      &                        & $\omega$                  & \xmark          & \xmark       & 62.3 $\pm$ 0.3          & 53.9 $\pm$ 0.2          & 75.2 $\pm$ 0.4          & 77.4 $\pm$ 0.1          & 67.2          \\
                                      &                        & $\omega$                  & \cmark          & \xmark       & 61.9 $\pm$ 0.4          & 52.6 $\pm$ 0.6          & 76.0 $\pm$ 0.8          & 77.5 $\pm$ 0.3          & 67.0          \\
                                      &                        & $\omega$                  & \cmark          & \cmark       & 62.3 $\pm$ 1.0          & 53.4 $\pm$ 0.3          & 76.0 $\pm$ 0.7          & 77.0 $\pm$ 0.1          & 67.2          \\
            \cmidrule{2-10}
            %   & Fishr                & $\omega$                    & \cmark       & \textbf{63.4} $\pm$ 0.8 & \textbf{54.2} $\pm$ 0.3 & \textbf{76.4} $\pm$ 0.3 & \textbf{78.5} $\pm$ 0.2 & \textbf{68.2} \\
                                      & \multirow{3}{*}{Fishr} & \multirow{3}{*}{$\omega$} & \xmark          & \xmark       & 61.8 $\pm$ 0.9          & 53.8 $\pm$ 0.4          & \textbf{76.6} $\pm$ 0.6 & 77.7 $\pm$ 0.2          & 67.5          \\
                                      &                        &                           & \cmark          & \xmark       & \textbf{63.6} $\pm$ 0.4 & 53.2 $\pm$ 0.5          & 75.4 $\pm$ 0.5          & 77.8 $\pm$ 0.3          & 67.5          \\
                                      &                        &                           & \cmark          & \cmark       & 63.4 $\pm$ 0.8          & \textbf{54.2} $\pm$ 0.3 & 76.4 $\pm$ 0.3          & \textbf{78.5} $\pm$ 0.2 & \textbf{68.2} \\
            \midrule
            \multirow{8}{*}{Training} & ERM                    & N/A                       & N/A             & N/A          & 61.3 $\pm$ 0.7          & 52.4 $\pm$ 0.3          & 75.8 $\pm$ 0.1          & 76.6 $\pm$ 0.3          & 66.5          \\
            \cmidrule{2-10}
                                      & \multirow{4}{*}{IGA}   & $\theta=(\phi, \omega)$   & \xmark          & \xmark       & 51.7 $\pm$ 1.3          & 49.3 $\pm$ 1.5          & 58.6 $\pm$ 7.1          & 69.0 $\pm$ 1.1          & 57.1          \\
                                      &                        & $\omega$                  & \xmark          & \xmark       & 61.9 $\pm$ 0.0          & 53.6 $\pm$ 0.9          & 75.7 $\pm$ 0.5          & 76.0 $\pm$ 0.1          & 66.8          \\
                                      &                        & $\omega$                  & \cmark          & \xmark       & 61.2 $\pm$ 0.1          & 52.2 $\pm$ 0.5          & 76.1 $\pm$ 0.2          & 77.2 $\pm$ 0.3          & 66.7          \\
                                      &                        & $\omega$                  & \cmark          & \cmark       & 61.7 $\pm$ 0.5          & 52.4 $\pm$ 0.7          & 75.9 $\pm$ 0.4          & 77.1 $\pm$ 0.2          & 66.8          \\
            \cmidrule{2-10}
            %   & Fishr                & $\omega$                    & \cmark       & \textbf{62.4} $\pm$ 0.5 & \textbf{54.4} $\pm$ 0.4 & \textbf{76.2} $\pm$ 0.5 & \textbf{78.3} $\pm$ 0.1 & \textbf{67.8} \\
                                      & \multirow{3}{*}{Fishr} & \multirow{3}{*}{$\omega$} & \xmark          & \xmark       & 63.8 $\pm$ 0.6          & 52.5 $\pm$ 0.5          & \textbf{76.7} $\pm$ 0.6 & 77.1 $\pm$ 1.0          & 67.5          \\
                                      &                        &                           & \cmark          & \xmark       & 62.2 $\pm$ 1.0          & 53.5 $\pm$ 0.2          & 76.6 $\pm$ 0.2          & 77.8 $\pm$ 0.4          & 67.5          \\
                                      &                        &                           & \cmark          & \cmark       & \textbf{62.4} $\pm$ 0.5 & \textbf{54.4} $\pm$ 0.4 & 76.2 $\pm$ 0.5          & \textbf{78.3} $\pm$ 0.1 & \textbf{67.8} \\
            \bottomrule
        \end{tabular}
    }
    \label{table:igahome}
\end{table}



==> tables/irm/cmnist_25.tex <==
% \begin{wraptable}[5]{hR!}{0.45\textwidth}
%     \vspace{-1.0em}
%     \caption{\textbf{Colored MNIST} results.}
%     \resizebox{1.0\linewidth}{!}{%

\begin{table}[!b]
    \vspace{-0.5em}
    \caption{\textbf{Colored MNIST results}. All methods re-use hyperparameters optimized for IRM.}
    \centering
    \resizebox{0.45\linewidth}{!}{%
    \begin{tabular}{c | c c c}
        \toprule
        Method & Train acc.     & Test acc.      & Gray test acc. \\
        \midrule
        ERM    & 86.4 $\pm$ 0.2 & 14.0 $\pm$ 0.7 & 71.0 $\pm$ 0.7 \\
        IRM    & 71.0 $\pm$ 0.5 & 65.6 $\pm$ 1.8 & 66.1 $\pm$ 0.2 \\
        V-REx  & 71.7 $\pm$ 1.5 & 67.2 $\pm$ 1.5 & 68.6 $\pm$ 2.2 \\
        Fishr  & 71.0 $\pm$ 0.9 & 69.5 $\pm$ 1.0 & 70.2 $\pm$ 1.1 \\
        \bottomrule
    \end{tabular}%
    }
    \label{table:cmnist_25}
\end{table}


==> tables/irm/cmnist_25_lateral.tex <==
\begin{wraptable}[8]{hR!}{0.45\textwidth}
    % \vspace{-1.0em}
    \caption{\textbf{Colored MNIST} results. All methods use hyperparameters optimized for IRM.}
    \resizebox{1.0\linewidth}{!}{%
    \centering
    \begin{tabular}{c  c c c}
        \toprule
        Method & Train acc.     & Test acc.      & Gray test acc. \\
        \midrule
        ERM    & 86.4 $\pm$ 0.2 & 14.0 $\pm$ 0.7 & 71.0 $\pm$ 0.7 \\
        IRM    & 71.0 $\pm$ 0.5 & 65.6 $\pm$ 1.8 & 66.1 $\pm$ 0.2 \\
        V-REx  & 71.7 $\pm$ 1.5 & 67.2 $\pm$ 1.5 & 68.6 $\pm$ 2.2 \\
        Fishr  & 71.0 $\pm$ 0.9 & 69.5 $\pm$ 1.0 & 70.2 $\pm$ 1.1 \\
        \bottomrule
    \end{tabular}%
    }
    \label{table:cmnist_25}
\end{wraptable}


==> tables/irm/cmnist_full.tex <==
\begin{table}[!htb]
    \caption{\textbf{Colored MNIST experiments}. All methods re-use hyperparameters optimized for IRM.}
    \centering
    \resizebox{0.70\textwidth}{!}{%
        \begin{tabular}{c | c c c | c c c}
            \toprule
                             & \multicolumn{3}{c|}{25\% label flipping} & \multicolumn{3}{c}{No label flipping}                                                                     \\
            \midrule
            Method           & Train acc.                               & Test acc.                             & Gray test acc. & Train acc.     & Test acc.      & Gray test acc. \\
            \midrule
            % Chance           & \multicolumn{3}{c|}{50}                  & \multicolumn{3}{c}{50}                                                                                             \\
            % Optimum          & \multicolumn{3}{c|}{75}                  & \multicolumn{3}{c}{100}                                                                                            \\
            Grayscale oracle & 75.5 $\pm$ 0.3                           & 72.5 $\pm$ 0.4                        & 72.5 $\pm$ 0.4 & 98.7 $\pm$ 0.0 & 97.8 $\pm$ 0.1 & 97.5 $\pm$ 0.1 \\
            \midrule
            ERM              & 86.4 $\pm$ 0.2                           & 14.0 $\pm$ 0.7                        & 71.0 $\pm$ 0.7 & 99.0 $\pm$ 0.0 & 91.8 $\pm$ 0.2 & 95.0 $\pm$ 0.4 \\
            IRM              & 71.0 $\pm$ 0.5                           & 65.6 $\pm$ 1.8                        & 66.1 $\pm$ 0.2 & 96.4 $\pm$ 0.2 & 82.2 $\pm$ 0.1 & 92.6 $\pm$ 0.2 \\
            V-REx            & 71.7 $\pm$ 1.5                           & 67.2 $\pm$ 1.5                        & 68.6 $\pm$ 2.2 & 97.1 $\pm$ 0.2 & 95.3 $\pm$ 0.4 & 94.1 $\pm$ 0.4 \\
            Fishr            & 71.0 $\pm$ 0.9                           & 69.5 $\pm$ 1.0                        & 70.2 $\pm$ 1.1 & 97.0 $\pm$ 0.2 & 95.3 $\pm$ 0.4 & 94.1 $\pm$ 0.4 \\
            \bottomrule
        \end{tabular}%
    }
    \label{table:cmnist}%
\end{table}%{tabular}

% gray
% Final train acc (mean/std across restarts so far):
% 0.75510997 0.0025607888
% Final test acc (mean/std across restarts so far):
% 0.72542 0.005198623
% Final gray test acc (mean/std across restarts so far):
% 0.72423995 0.0029059285

% Final train acc (mean/std across restarts so far):
% 0.98713195 0.00022683998
% Final test acc (mean/std across restarts so far):
% 0.97835 0.00052392
% Final gray test acc (mean/std across restarts so far):
% 0.97464 0.0010800108

% ERM
% Final train acc (mean/std across restarts so far):
% 0.989676 0.00026469506
% Final test acc (mean/std across restarts so far):
% 0.91775 0.0021058305
% Final gray test acc (mean/std across restarts so far):
% 0.95043993 0.0041146553
% Final train acc (mean/std across restarts so far):
% 0.863476 0.0021055692
% Final test acc (mean/std across restarts so far):
% 0.13978001 0.0067230635
% Final gray test acc (mean/std across restarts so far):
% 0.71017 0.007419707

% => IRM
% Final train acc (mean/std across restarts so far):
% 0.709754 0.004756992
% Final test acc (mean/std across restarts so far):
% 0.65639997 0.018081106
% Final gray test acc (mean/std across restarts so far):
% 0.66075 0.021708393
% Final train acc (mean/std across restarts so far):
% 0.9639179 0.0021445584
% Final test acc (mean/std across restarts so far):
% 0.82194996 0.013370054
% Final gray test acc (mean/std across restarts so far):
% 0.92635995 0.017597286
% => Rex
% Final train acc (mean/std across restarts so far):
% 0.71726197 0.015138928
% Final test acc (mean/std across restarts so far):
% 0.67156994 0.015151371
% Final gray test acc (mean/std across restarts so far):
% 0.68614 0.021597888

% Final train acc (mean/std across restarts so far):
% 0.9706559 0.0022299953
% Final test acc (mean/std across restarts so far):
% 0.95283 0.0038984746
% Final gray test acc (mean/std across restarts so far):
% 0.94146997 0.004081438

% => Fishr
% Final train acc (mean/std across restarts so far):
% 0.70959604 0.009424484
% Final test acc (mean/std across restarts so far):
% 0.69459 0.009932211
% Final gray test acc (mean/std across restarts so far):
% 0.70242995 0.011290974
% Final train acc (mean/std across restarts so far):
% 0.970432 0.0023718535
% Final test acc (mean/std across restarts so far):
% 0.95298994 0.0040908344
% Final gray test acc (mean/std across restarts so far):
% 0.94079 0.0037911658


==> tables/irm/cmnist_hessian.tex <==
% \begin{wraptable}[16]{hR!}{0.36\textwidth}
%     \centering
%     % \vspace{-7em}
%     % \caption{\textbf{Colored MNIST dynamics}, where $\mathcal{E}=\{90\%,80\%\}$. Details in Appendix \ref{appendix:cmnistdetails}.
%     % At epoch 190, $\lambda$ strongly steps up: then the Fishr regularization from Eq.~\ref{eq:fishrreg} matches the domain-level gradients covariances ($\mC_{90\%}$ and $\mC_{80\%}$, blue line).
%     % Critically, Fishr also reduces the distance between the two domain-level Hessians ($\mH_{90\%}$ and $\mH_{80\%}$, green line).}
%     \caption{
%         \textbf{Hessians comparison} across the two training domains $\mathcal{E}=\{90\%,80\%\}$ in Colored MNIST \textbf{at convergence}, for ERM and Fishr strategies.
%         Details in Appendix \ref{appendix:hessianmatching}. Fishr regularization matches domain-level gradient covariances ($\mC_{90\%}$ and $\mC_{80\%}$) and most importantly also matches Hessians ($\mH_{90\%}$ and $\mH_{80\%}$) diagonals.}
%     % \vspace{-0.5em}
%     \resizebox{\linewidth}{!}{%
%         \begin{tabular}{c c c}
%             % \toprule
%             %                                                & ERM                    & Fishr                 \\
%             % \midrule
%             % $\left\|\mC_{90\%}-\mC_{80\%}\right\|_{F}^{2}$ & 0.003133662207983434   & 2.226968513241445e-06 \\
%             % % \midrule
%             % $\left\|\mH_{90\%}-\mH_{80\%}\right\|_{F}^{2}$ & 0.00025846528296824545 & 2.026419122103107e-06 \\
%             % % $|\left\|\mH_{90\%}\right\|_{F}^{2} -\left\|\mH_{80\%}\right\|_{F}^{2}|^{2}$ & 2.1760304480267224e-05 & 4.1325527837532406e-07 \\
%             % % $\cos\left(\mH_{90\%}, \mH_{80\%}\right)}$                                   & 0.9999978721141816     & 0.9999959528446197     \\
%             % \toprule
%             % Method & $\left\|\operatorname{Diag}\left(\mC_{90\%}-\mC_{80\%}\right)\right\|_{F}^{2}$ & $\left\|\operatorname{Diag}\left(\mH_{90\%}-\mH_{80\%}\right)\right\|_{F}^{2}$ \\
%             % \midrule
%             % ERM    & $3 * 10^{-3}$                                                                  & $3 * 10^{-4}$                                                                  \\
%             % % \midrule
%             % Fishr  & $2 * 10^{-6}$                                                                  & $2 * 10^{-6}$                                                                  \\
%             % $|\left\|\mH_{90\%}\right\|_{F}^{2} -\left\|\mH_{80\%}\right\|_{F}^{2}|^{2}$ & 2.1760304480267224e-05 & 4.1325527837532406e-07 \\
%             % $\cos\left(\mH_{90\%}, \mH_{80\%}\right)}$                                   & 0.9999978721141816     & 0.9999959528446197     \\
%             \toprule
%                                                                                            & ERM             & Fishr           \\
%             \midrule
%             $\left\|\operatorname{Diag}\left(\mC_{90\%}-\mC_{80\%}\right)\right\|_{F}^{2}$ & $3.1 \times 10^{-3}$ & $2.2 \times 10^{-6}$ \\
%             % \midrule
%             $\left\|\operatorname{Diag}\left(\mH_{90\%}-\mH_{80\%}\right)\right\|_{F}^{2}$ & $2.6 \times 10^{-4}$ & $2.0 \times 10^{-6}$ \\
%             \bottomrule%
%         \end{tabular}%
%     }%
%     \label{table:hessianermfishr}%
% \end{wraptable}%%


==> tables/oracle/db_all_oracle_poster.tex <==
% Table 2:
\begin{table*}[t]%
    \caption{\textbf{DomainBed benchmark}. We format \textbf{first}, \underline{second} and \textcolor{gray}{worse than ERM} results.}%
    \centering
    \adjustbox{width=1.0\textwidth}{
        \begin{tabular}{ll|cccccccc|c}
            \toprule
            \multirow{2}{*}{\textbf{Algo.}} & \multirow{2}{*}{\textbf{Invariance}} & \multicolumn{8}{c|}{Acc. $\uparrow$}    & \multicolumn{1}{c}{Rank $\downarrow$}                                                                                                                                                                                                                                                                                                                                                            \\
                                                & &\textbf{cMNIST}                               & \textbf{rMNIST}                               & \textbf{VLCS}                                 & \textbf{PACS}                                 & \textbf{OHome}                           & \textbf{TerraI}                             & \textbf{DNet}                            & \textbf{Avg}           & \textbf{Avg}      \\
            \midrule
            ERM                 & \xmark                & 57.8                    & 97.8                    & 77.6                    & 86.7                    & 66.4                    & \underline{53.0}                    & 41.3                    & 68.7                   & 9.1             \\
            \midrule
            CORAL                          & \multirow{2}{*}{Features}     & 58.6                    & \textbf{98.0}        & 77.7                    & \underline{87.1}                    & \textbf{68.4}           & \textcolor{gray}{52.8}  & \underline{41.8}        & \underline{69.2}       & \underline{4.6}  \\
            DANN                               & & \textcolor{gray}{57.0}  & \underline{97.9}                    & \textbf{79.7}        & \textcolor{gray}{85.2}  & \textcolor{gray}{65.3}  & \textcolor{gray}{50.6}  & \textcolor{gray}{38.3}  & \textcolor{gray}{67.7} & \textcolor{gray}{11.9}   \\
            \midrule
            IRM                                 & \multirow{2}{*}{Predictors}& \underline{67.7}        & \textcolor{gray}{97.5}  & \textcolor{gray}{76.9}  & \textcolor{gray}{84.5}  & \textcolor{gray}{63.0}  & \textcolor{gray}{50.5}  & \textcolor{gray}{28.0}  & \textcolor{gray}{66.9} & \textcolor{gray}{14.7}  \\
            V-REx                               && 67.0                    & \underline{97.9}                    & 78.1                    & \textbf{87.2}           & \textcolor{gray}{65.7}  & \textcolor{gray}{51.4}  & \textcolor{gray}{30.1}  & \textcolor{gray}{68.2} & 7.7                        \\
            \midrule
            Fish                            & \multirow{2}{*}{Gradients}    & 61.8                    & \underline{97.9}                    & 77.8                    & \textcolor{gray}{85.8}  & \textcolor{gray}{66.0}  & \textcolor{gray}{50.8}  & \textbf{43.4}           & 69.1                   & 8.4               \\
            \textbf{Fishr}                       &        & \textbf{68.8}           & 97.8                    & \underline{78.2}                    & 86.9                    & \underline{68.2}        & \textbf{53.6}        & \underline{41.8}        & \textbf{70.8}          & \textbf{3.9}           \\
            \bottomrule
        \end{tabular}
    }
    \label{table:db_all_oracle}%
\end{table*}





==> tables/oracle/tmp.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Benchmarks \& Implementation}

\paragraph{Benchmarks \& Metrics} We evaluate our model on CIFAR100 \cite{krizhevskycifar100}, ImageNet100 and ImageNet1000 \cite{deng2009imagenet} (datasets description in the supplementary materials) under different settings, where for each the number of new classes seen per step is different.
The standard continual scenario in ImageNet has 10 steps: thus we add 10 new classes per step in ImageNet100, and 100 new classes per step in ImageNet1000.
In CIFAR100, we compare performances on 10 steps (10 new classes per step), 20 steps (5 new classes per step), and 50 steps (2 new classes per step).
In addition to the top-1 accuracy, we also compare the top-5 accuracy on ImageNet.
We report the ``\textit{Avg}'' accuracy which is the average of the accuracies after each step as defined by \cite{rebuffi2017icarl}.
We also report the final accuracy after the last step (``\textit{Last}'').
Finally ``\textit{\#P}'' denotes the parameter count in million after the final step.

\input{tables/transf_archi}
\input{tables/imagenet}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{images/imagenet100.png}
    \caption{\textbf{Performance evolution on ImageNet100}. The top-5 accuracy (\%) is reported after learning each task. Our model DyTox (in \textbf{\textcolor{red}{red}}) surpasses significantly most baselines, and is of equal performance as the complex DER that uses pruning with setting-specific hyperparameters. \alex{remettre les poids dans la FIgure 1, non ?}}
    \label{fig:imagenet100}
\end{figure}
\paragraph{Implementation details} As highlighted in \autoref{tab:archi}, our network architecture has the same structure across tasks. Specifically, we use 5 Self-Attention Blocks (SABs), 1 Task-Attention Block (TAB). All 6 have an embedding dimension of 384 and 12 attention heads.
We designed our transformer shallow (6 blocks) to have a comparable parameters count to other baselines, but also made it wider than usual "tiny" models \cite{dosovitskiy2020vit,touvron2021deit,touvron2021cait} (384d).
We tuned these hyperparameters for CIFAR100 10 steps, and then kept them fixed for all other settings, ImageNet included.
We use the attention with spatial prior introduced by ConViT \cite{dascoli2021convit} for all SABs which allows training transformers on a small dataset (like CIFAR) without pretraining on large datasets or complex regularizations. We use for all models (baselines included) 2,000 \alex{c'est standard comme chiffre? citation} images of rehearsal memory for CIFAR100 and ImageNet100, and 20,000 images for ImageNet1000.
The implementations of the continual scenarios are provided by Continuum \cite{douillardlesort2021continuum} and our \alexd{code}{implementation, code est repeté juste apres} is based on the DeiT \cite{touvron2021deit} code base which itself uses extensively the timm library \footnote{available at \url{http://github.com/rwightman/pytorch-image-models/}}. We'll release publicly our code to facilitate the reproduction of our results \alex{important: faudrait faire un repo anonym. Même donner l'url dans l'abstract/intro. Ca changera des DER}. The full implementation details can be found in the supplementary materials.

\paragraph{Baselines}
\alexd{DyTox has slightly more parameters on ImageNet than on CIFAR (11.014M vs 10.687M) for an equal amount of steps because more patch tokens exist for the former dataset resulting in bigger learned positional embeddings in the tokenizer}{à mettre dans implementation details}.
ImageNet data is more complex than CIFAR (image sizes are 32$\times$32 vs 224$\times$224) and the image diversity is significantly higher
DER proposed a pruning method to reduce that amount to an acceptable level; unfortunately, this pruning required a different hyperparameter tuning for each setting. We denote by a $^\dagger$ the DER with setting-specific pruning, and \textit{w/o P} for the DER without pruning. Simple-DER also uses pruning but without the need of hyperparameter tuning.
As a result DER struggles to scale and its pruning is less efficient than on CIFAR (detailed later).
%Our main concurrent, DER, has less significant gain in this 10-steps ImageNet100 compared to the 10-steps CIFAR100, and their pruning procedure is also less effective (4.96M vs 7.67M).


\input{tables/cifar100_b0}

\begin{figure*}[t!]
\centering
  \includegraphics[width=0.9\linewidth]{images/cifar.png}
    \caption{Accuracy for each step on the CIFAR100 dataset. \textbf{Left} is evaluated with 10 steps, \textbf{middle} with 20 steps, and \textbf{right} 50 steps.}
\label{fig:increment_cifar}
\end{figure*}

\subsection{Quantitative results}


\paragraph{ImageNet100}
We report performances in \autoref{tab:imagenet} on the complex ImageNet dataset.
In ImageNet100, DyTox reaches 67.76\% and outperforms the pruned DER$^\dagger$ by +1.7 percentage points (p.p.) in ``Last'' accuracy. Though, DyTox and DER somehow performs similarly ``Last'' accuracy on this setup, as highlighted in the performance evolution displayed in \autoref{fig:imagenet100}.

\paragraph{ImageNet1000}
Yet, on the larger-scale ImageNet1000, DyTox systematically performs best on all metrics despite having lower parameter count.
Specifically, DyTox reaches 71.51\% in average top-1 accuracy, and 61.28\% in ``Last'' accuracy. This outperforms the previous state-of-the-art DER, without without pruning (68.84\% in ``Avg'', 60.16 in ``Last'') with 10 ResNet18 in parallel and 61.6m parameters.
Compared to the pruned DER$^\dagger$, DyTox has a +4.8 p.p. in top-1 and a +1.7 p.p. in top-5 for the ``Avg'' accuracy.
All models evolutions on ImageNet1000 are illustrated in \autoref{fig:imagenet1000}: DyTox constantly surpasses previous state-of-the-art models despite having comparable performance at the first step.
This shows that DyTox is able to scale correctly despite learning ten times more classes, while handling seamlessly the parameter growth.
Indeed, the parameter count between ImageNet100 and ImageNet1000 doesn't change: in contrast, DER doubles in size (14.52M \textit{vs.} 7.67M).

\paragraph{CIFAR100} We report in \autoref{tab:cifar100-b0} results for all approaches on CIFAR100.
The more steps there are, the larger is the forgetting and thus the lower is the performance.
%RPSNet \cite{rajasegaran2019rpsnet} and DER \cite{yan2021der} have a large number of parameters because of their dynamic strategy.
% https://github.com/Rhyssiyan/DER-ClassIL.pytorch/issues/4#issuecomment-865853428
%This is unrealistic because in a true continual learning, we aren't supposed to know the number of future classes and thus the same hyperparameters should be applied to all settings of a same dataset.
% (see \autoref{sec:memory_overhead})
Furthermore, the memory overhead per task is very small: our base network has 10.684M parameters, 10.687M with 10 class tokens, and 10.702M with 50 class tokens: that is a vector of size $+\mathbb{D}$ per task.
In our case, $\mathbb{D}=384$ and the base model has $\sim11$M parameters, thus the overhead in memory is only of $+0.03\%$ per task. Given the challenging setting of CIFAR100 with 50 tasks, our memory overhead is still small ($+1.74\%$).
In every setting, DyTox is close to ``DER without pruning'' for much fewer parameters (up to 26x less) and significantly above other baselines (up to +25\% in ``Last'' accuracy in 50 steps).
Those settings are also displayed in \autoref{fig:increment_cifar}, where model performances are displayed after every step.
Our dynamic strategy doesn't require any complex pruning: this is possible by sharing early layers.
%  and extracting class-agnostic features \cite{olah2017feature}


\paragraph{Improved Training Procedure} To bridge the gap between DyTox and DER on CIFAR100, we propose an efficient training procedure for continual learning.
Using MixUp \cite{hingyi2018mixup}, we linear interpolate new samples with existing samples. The interpolation factor is sampled $\lambda \sim \operatorname{Beta}(\alpha, \alpha)$: the pixels of two images are mixed ($x = \lambda x_1 + (1 - \lambda) x_2$) as their labels ($y = \lambda y_1 + (1 - \lambda) y_2$). MixUp was shown to have two main effects: (1) it diversifies the training images and thus enlarges the training distribution on the vicinity of each training sample \cite{chapelle2001vicinalrisk} and (2) it improves the network calibration \cite{guo2017miscalibration,thulasidasan2019mixupcalibration}, reducing the overconfidence in recent classes.
Thus MixUp has shared motivation with the use of the sigmoid activation.
When DyTox is combined with this MixUp procedure, nicknamed as DyTox+, we significantly improve the state of the art in ``Avg'' accuracy in all three settings of \autoref{tab:cifar100-b0}.


\paragraph{Training procedure introspection}
Critically, MixUp really reduces catastrophic forgetting and does not just improve raw performances.
This is shown in \autoref{tab:training_plus}, where we compare DyTox \textit{vs.} DyTox+ strategies on CIFAR100.
While MixUp only slightly improves by 1.39 p.p. the accuracy in joint learning (no continual, 1 step), MixUp greatly improves by 4.75 p.p. in the 50 steps continual scenario.
To further illustrate this, we also report the Chaudhry's forgetting \cite{chaudhry2018riemannien_walk} which compares how performances dropped compared to previous steps.
MixUp reduces this forgetting measure by 1.65 p.p..

\label{sec:ablations}
\paragraph{Model ablations:} We ablate the importance of the different components of DyTox in \autoref{tab:ablation} on the 50 steps setting of CIFAR100.
The baseline formulation proved to be already efficient to handle forgetting.
We further add a naive knowledge distillation \cite{hinton2015knowledge_distillation} and a finetuning \cite{castro2018end_to_end_inc_learn,hou2019ucir,douillard2020podnet,yan2021der} applied after each task on a balanced set of new data and rehearsal data.
Finally, our DyTox strategy exploits directly the very nature of transformers (separated task information from the pixels information) to tackle catastrophic forgetting: it is made of three components: (1) a task token expansion, (2) a divergence classifier, and (3) independent classifiers. All three greatly improve over the baseline transformer ($42.21\% \rightarrow 52.34\%$ in ``All'') while having almost no memory overhead. The independent classifiers with the sigmoid activations reduce the Chaudhry's forgetting \cite{chaudhry2018riemannien_walk} by more than 8 p.p..


\input{tables/ablations}

\input{tables/plus}


\label{sec:comp_over}
\alex{à mettre dans la partie model}
\paragraph{Computational Overhead:} The vast majority of the computation, done in the SABs, is shared among all tasks. The dynamical component of our model is located at the ultimate TAB. Moreover, the Task-Attention, contrary to the Self-Attention, has a time complexity linear in terms of tokens and not quadratic further reducing the time overhead to an acceptable amount. Overall, for each new task, one forward pass takes $2.24\%$ more time w.r.t the base transformer speed.

%\input{tables/sam}

%\input{tables/aug}
%\input{tables/ens_ablation}
%\input{tables/archi}
%\input{tables/old_sam}
%\input{tables/transf}

